Safeguarding adaptive methods: global convergence of Barzilai-Borwein and other stepsize choices

Leveraging on recent advancements on adaptive methods for convex minimization problems, this paper provides a linesearch-free proximal gradient framework for globalizing the convergence of popular stepsize choices such as Barzilai-Borwein and one-dimensional Anderson acceleration. This framework can cope with problems in which the gradient of the differentiable function is merely locally H\"older continuous. Our analysis not only encompasses but also refines existing results upon which it builds. The theory is corroborated by numerical evidence that showcases the synergetic interplay between fast stepsize selections and adaptive methods.

==> TeX/Preamble.tex <==
\makeatletter

	\IEEEoverridecommandlockouts
	\overrideIEEEmargins

%% Packages
	\let\labelindent\relax
	\let\NAT@parse\undefined
	\PassOptionsToPackage{capitalize,nameinlink}{cleveref}
	\usepackage[
		noload={caption,subcaption},
	]{myPreamble}
	\pgfplotsset{compat=1.18}
	\hypersetup{hypertexnames=false}




	\newcommand{\arXivLink}[1]{\href{https://arxiv.org/abs/#1}{arXiv:\allowbreak#1}}


	\crefformat{section}{#2\S #1#3}
	\Crefformat{section}{#2Section #1#3}
	\renewcommand{\enumeratelabeli}{\arabic*}
	\renewcommand{\refenumeratelabeli}{{\it(\arabic*)}}
	\renewcommand{\enumerateSuffixi}{.}

	\renewcommand{\proofitemizelabeli}{\(\diamondsuit\)}
	\newlist{claims}{enumerate}{1}
	\setlist[claims,1]{
		label={\(\diamondsuit\)\,\it Claim \ref*{\currentlabel}(\alph*):},
		ref={\ref*{\currentlabel}(\alph*)},
		topsep=0pt,
		partopsep=0pt,
		parsep=0pt,
		itemsep=1ex,
		wide=0pt,
		leftmargin=0pt,
		labelindent=0.25cm,
	}
	\newlist{claims*}{enumerate}{1}
	\setlist[claims*,1]{
		label={\it Contradiction claim \oldstylenums{\arabic*}$^*$:},
		ref={\oldstylenums{\arabic*}$^*$},
		partopsep=0pt,
		parsep=0pt,
		itemsep=3pt,
		wide,
		labelindent=0pt,
	}

	\RegisterTheoremName{claimsi}{Claim}

	\Crefname{claimsi}{Claim}{Claims}

	\newcommand{\algnamefont}{\sf}
	\renewcommand{\AA}{{\algnamefont AA}}
	\newcommand{\adaPBB}{{\algnamefont adaPBB}}
	\newcommand{\adaPG}{\text{\algnamefont adaPG$^{\rp,\frac{\rp}{2}}$}}
	\newcommand{\AdaPG}{\text{\algnamefont AdaPG$^{\rp,\frac{\rp}{2}}$}}
	\newcommand{\BB}{\@ifstar\@@BB\@BB}
	\newcommand{\@BB}{\text{\algnamefont BB\textsuperscript{long}}}
	\newcommand{\@@BB}{\text{\algnamefont BB\textsuperscript{short}}}
	\newcommand{\fast}{{\algnamefont fast}}
	\newcommand{\safe}{{\algnamefont safe}}

	\let\@innprod\@@innprod

	\xpatchcmd\algorithmic{\leftmargin\labelwidth}{\leftmargin=7pt}{}{}


%% k, k+1 commands
	\newcommand{\newvark}{\@ifstar\@@newvark\@newvark}
	\newcommand{\@newvark}[2]{\newcommand #1{\@ifstar{#2_{k+1}}{#2_k}}}
	\newcommand{\@@newvark}[2]{\newcommand #1{\@ifstar{#2^{k+1}}{#2^k}}}

	\newcommand{\renewsymbol}[2]{\let#2#1\renewcommand #1{\text{\huge\red$#2$}}}
	\renewsymbol{\gamma}{\gam}
	\renewsymbol{\lambda}{\lamb}
	\renewsymbol{\pi}{\rp}

	\newcommand{\x}{x}
	\newcommand{\U}{\mathcal U^{\rp}}
	\renewcommand{\rp}{q}

	\def\c_#1{c_{{#1},\q}}
	\def\l_#1{\ell_{{#1},\q}}
	\def\L_#1{L_{{#1},\q}}
	\def\lam_#1{\lamb_{{#1},\q}}

	\newvark{\ck}{\c}
	\newvark{\gamk}{\gam}
	\newvark{\Hk}{H}
	\newvark{\lamk}{\lam}
	\newvark{\lk}{\l}
	\newvark{\Lk}{\L}
	\newvark{\rhok}{\rho}
	\newvark{\Uk}{\U}

	\newvark*{\xk}{\x}


%% Symbols
	\let\oldnabla\nabla
	\renewcommand{\nabla}{\@ifstar{\widetilde{\oldnabla}}{\oldnabla}}
	\DeclareMathOperator{\diam}{diam}
	\newcommand{\q}{\nu}
	\renewsymbol{\|}{\oldvert}
	\DeclarePairedDelimiter\norm{\lVert}{\rVert}
	\DeclarePairedDelimiter\abs{\lvert}{\rvert}

	\newcommand{\K}{\@ifstar{K^{\downarrow}}{K^{\uparrow}}}


	\pgfplotsset{compat=1.16} %pgfplots的版本
	\usepgfplotslibrary{groupplots}

	%Axis
	\pgfplotsset{
		filter discard warning = false,
		myaxis/.style = {
			xmin = 0,     %图表上下限
			grid = major, %网格线
			grid style = {dashed, line width = .1pt, draw = gray!10}, %网格线格式 dashed虚线  line width = .1pt 表示网格线宽度0.1  draw = gray!10 表示浅(10%)灰色
			major grid style = {line width = .2pt, draw = gray!50}, %主要网格线样式 已将grid style覆盖
			legend style = {at = {(1,1)},  font = {\algnamefont},  opacity=0.65},%anchor = north east, %legend style图例的样式 at={(1,1)} 图例的坐标 通常是右上角 anchor指定哪个角落在at的位置 font 图例文字的字体大小 scriptsize表示比正文小一些 opacity = 0.5 代表图例的不透明度 会透明一些
			legend cell align={left},
			scaled ticks=false, tick label style={/pgf/number format/fixed},
% 			label style = {font=\tiny},
% 			tick label style={font=\tiny},
% 			title style = {font=\tiny},
		},
	}

	%% Lines
	\pgfplotsset{
		plotline/.style 2 args = {
			thick, % 从细到粗有 ultra thin, very thin, thin, semithick, thick, very thick, ultra thick 也可以通过line width =2pt 的方式来指定线宽
			mark = {#1}, % 多种标记样式 * 星号 + 加号 x 叉号 o 圆圈 square 正方形 triangle 三角形 diamond 菱形 pentagon 五边形 none 无标记
			color = {#2}, % 预定义颜色 black white red green blue cyan magenta yellow gray darkgray lightgray brown lime olive orange pink purple teal violet 也可以用xcolor自定义颜色 例如 gray！50  red!70!blue...
			mark size = 2pt, %标记大小
			mark options = {solid}, %标记实心
			mark repeat = 25, %每隔5个数据点重复一次标记
			mark phase = 1, %从第一个书据点开始标记
			line width = 0.75pt,
		},
		plotline*/.style 2 args = {
			plotline = {#1}{#2},
			dashed,         %线条变成虚线
		},
		AdaPBB/.style = {%
			plotline* = {none}{blue},
			line width = 1.5pt,
		},
		AdaPG/.style = {%black white red green blue cyan magenta yellow gray darkgray lightgray brown lime olive orange pink purple teal violet
			plotline = {none}{black},
			line width = 1.5pt,
		},
		AdaPG_BBlong/.style = {%
			plotline = {diamond}{Green},
		},
		AdaPG_BBshort/.style = {%
			plotline = {o}{Orange},
		},
		AdaPG_Martinez/.style ={%
			plotline ={triangle}{olive},
		},
		AdaPG_LNSE/.style = {%
			plotline = {+}{teal},
		},
		AdaPG_AA/.style = {
			plotline = {square}{purple},
% 			mark size = 2.7pt,
% 			mark options = {dashed},
		},
	}

\makeatother


==> TeX/Text/Conclusions.tex <==
This work demonstrates that a minimal modification in the update rule of adaptive schemes
{\Red Future work: exploit variable parameters \(\rp_k\) and \(r_k\) in \cite{latafat2023convergence}}
Moreover, the flexibility of the propsed framework in accommodating virtually arbitrary stepsizes motivates the quest for new fast stepsize selections, which we believe is another interesting problem for future work.

